Does Feasibility Matter? Understanding the Impact of Feasibility on Synthetic Training Data

With the development of photorealistic diffusion models, models trained in part or fully on synthetic data achieve progressively better results. However, diffusion models still routinely generate images that would not exist in reality, such as a dog floating above the ground or with unrealistic texture artifacts. We define the concept of feasibility as whether attributes in a synthetic image could realistically exist in the real-world domain; synthetic images containing attributes that violate this criterion are considered infeasible. Intuitively, infeasible images are typically considered out-of-distribution; thus, training on such images is expected to hinder a model's ability to generalize to real-world data, and they should therefore be excluded from the training set whenever possible. However, does feasibility really matter? In this paper, we investigate whether enforcing feasibility is necessary when generating synthetic training data for CLIP-based classifiers, focusing on three target attributes: background, color, and texture. We introduce VariReal, a pipeline that minimally edits a given source image to include feasible or infeasible attributes given by the textual prompt generated by a large language model. Our experiments show that feasibility minimally affects LoRA-fine-tuned CLIP performance, with mostly less than 0.3% difference in top-1 accuracy across three fine-grained datasets. Also, the attribute matters on whether the feasible/infeasible images adversarially influence the classification performance. Finally, mixing feasible and infeasible images in training datasets does not significantly impact performance compared to using purely feasible or infeasible datasets.

==> sec/6_acknowledgement.tex <==
\section{Acknowledgments}
Jae Myung Kim thanks the International Max Planck Research School for Intelligent Systems (IMPRS-IS)
and the European Laboratory for Learning and Intelligent Systems (ELLIS) PhD programs for support.

% This work was supported by the ERC (853489 - DEXIM) and the BMBF (Tübingen AI Center, FKZ: 01IS18039A). 
% Cordelia Schmid would like to acknowledge the support by the K\"orber European Science Prize. Also, the authors gratefully acknowledge the Gauss Centre for Supercomputing e.V. (www.gauss-centre.eu) for funding this project by providing computing time on the GCS Supercomputer JUWELS at Jülich Supercomputing Centre (JSC).


==> tabs/main_result2.tex <==
\begin{table}[h]
\centering
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{c|cc|ccc|c}
\toprule
& \textbf{R} & \textbf{S} & \textbf{Pets~\cite{pets}} & \textbf{AirC~\cite{aircraft}} & \textbf{Cars~\cite{cars}} & \textbf{Avg} \\ 
\midrule
0-shot Base 
   & & &
  91.0 & 23.8 & 63.2 & 59.3 \\ 

\midrule
Back. &  & \rc &
  95.2 & 86.6 & 93.8 & 91.9 \\
Color & & \rc &
  94.1 & 81.9 & 92.1 & 89.4 \\
Text. &
  \multirow{-3}{*}{} & \multirow{-3}{*}{\rc \ding{51}} &
  92.8 & 82.0 & 91.8 & 88.9 \\ 

\hline 
Back. & \rc & \rc &
  95.3 & 88.0 & 93.6 & 92.3 \\
Color & \rc & \rc &
  95.0 & 83.4 & 92.8 & 90.4 \\
Text. &
  \multirow{-3}{*}{\rc \ding{51}} & \multirow{-3}{*}{\rc \ding{51}} &
  95.2 & 83.8 & 92.6 & 90.5 \\ 
  
\hline
Real &
   & \rc \ding{51} &
  95.2 & 84.5 & 92.6 & 90.8 \\ 
  
\bottomrule
\end{tabular}%
}
\vspace{-0.5em}
\caption{The top-1 performance results using the full training set combined with a balanced mix of feasible and infeasible synthetic data, with training setups including synthetic-only and synthetic + full real data. All results use synthetic images set to five times the number of real images.}
\label{tab: main2}
\vspace{-1.0em}
\end{table}


